Peer Grading in a Course on Algorithms and Data Structures: Machine Learning Algorithms do not Improve over Simple Baselines

Peer grading is the process of students reviewing each others' work, such as homework submissions, and has lately become a popular mechanism used in massive open online courses (MOOCs). Intrigued by this idea, we used it in a course on algorithms and data structures at the University of Hamburg. Throughout the whole semester, students repeatedly handed in submissions to exercises, which were then evaluated both by teaching assistants and by a peer grading mechanism, yielding a large dataset of teacher and peer grades. We applied different statistical and machine learning methods to aggregate the peer grades in order to come up with accurate final grades for the submissions (supervised and unsupervised, methods based on numeric scores and ordinal rankings). Surprisingly, none of them improves over the baseline of using the mean peer grade as the final grade. We discuss a number of possible explanations for these results and present a thorough analysis of the generated dataset.

==> ules_latex_colors.tex <==

\ifx\ulesred\undefined
\typeout{DEFINING COLORS}
\usepackage{color}

% defining colors: 
\definecolor{ulesred}{rgb}{0.7,0,0}
\newcommand{\ulesred}{\color{ulesred}}
\newcommand{\ur}{\ulesred}

\definecolor{darkgreen}{rgb}{0,0.5,0.2}
\newcommand{\darkgreen}{\color{darkgreen}}
\newcommand{\ulesgreen}{\color{darkgreen}}
\newcommand{\ug}{\ulesgreen}

\definecolor{verylightgray}{gray}{0.85} 
\newcommand{\lightgray}{\color{verylightgray}} % to be used on paper 
\definecolor{mediumgray}{gray}{0.5} 
\newcommand{\mediumgray}{\color{mediumgray}} % to be used on slides
\definecolor{darkgray}{gray}{0.4} 
\newcommand{\darkgray}{\color{darkgray}} % to be used on slides

\newcommand{\gray}{\mediumgray}
\newcommand{\grey}{\gray}
\newcommand{\printgray}{\lightgray} % to be used on paper 
\newcommand{\slidegray}{\mediumgray} % to be used on slides



\definecolor{lavender}{cmyk}{0,0.5,0,0}
\newcommand{\lavender}{\color{lavender}}

\definecolor{darkblue}{rgb}{0,0,0.5}
\newcommand{\darkblue}{\color{darkblue}}


\definecolor{orange}{rgb}{1,0.5,0}
\newcommand{\orange}{\color{orange}}
\else

\fi


% defining shortcuts to standard colors:  
\ifx\black\undefined
\newcommand{\black}{\color{black}}
\fi

\ifx\blue\undefined
\newcommand{\blue}{\color{blue}}
\fi

\ifx\red\undefined
\newcommand{\red}{\color{red}}
\fi

\ifx\green\undefined
\newcommand{\green}{\color{green}}
\fi

\ifx\white\undefined
\newcommand{\white}{\color{white}}
\fi 


\ifx\magenta\undefined
\newcommand{\magenta}{\color{magenta}}
\fi 



==> ules_latex_defaults.tex <==
% ------------------------------------------------------------
% ------------------------------------------------------------

% Ule's latex default settings
% simply include per 'input' in the current latex file 

\typeout{Using Ule's latex defaults!}

% ------------------------------------------------------------
% ------------------------------------------------------------

% ------------------------------------------------------------
% packages:
% ------------------------------------------------------------

% mathematical stuff: 
\usepackage{amssymb}
\usepackage{amsmath}
\allowdisplaybreaks[3] % page breaks inside eqnarray, see ams doku  
\usepackage{bbold} % used in definition of \charfct 
%\usepackage[mathcal]{euscript} % curlier version of mathcal symbols

% for figures: 

\usepackage{flafter} % no figure before the place it is defined 
\PassOptionsToPackage{pdftex}{graphicx} %flafter loads graphicx, but
                                %without option. will lead to option
                                %clash with graphicx package unless
                                %this line is put in ... 

\usepackage[pdftex]{graphicx}
%\DeclareGraphicsExtensions{.pdf}


% for the layout and general stuff

% put in paper directly if necessary
% \usepackage{geometry}
% \geometry{verbose,a4paper,tmargin=2cm,bmargin=3cm,lmargin=3cm,rmargin=3cm}

\usepackage{fancyhdr} % for nice head-and footlines
\usepackage{ifthen} % for \ifthenelse
\usepackage{layout} 
\usepackage{xspace}% for nice spaces after macros 
\usepackage{afterpage}% to flush floats nicely; use
                      % \afterpage{\clearpage} to flush all figures
                      % but without starting a new page
\usepackage{url} 
\usepackage{textcomp} %for the euro symbol; \texteuro

% for smileys and lightnings: 
\usepackage{wasysym} 
%has to be included
% after amsmath because of a bug! 
% for other wasysym stuff see below. 

% to show labels:
%\usepackage[notref,notcite]{showkeys_tiny}

% ------------------------------------------------------------
% Language - force german or english: 
% ------------------------------------------------------------

%\usepackage[english]{babel}
%\usepackage{german}
\usepackage[latin1]{inputenc} %for 8bit-umlaute produced by emacs

% ------------------------------------------------------------
% bib:
% put this in the article directly, causes confusion when used to
% produce journal papers
% ------------------------------------------------------------


%%\usepackage[round,comma]{natbib}
%%\bibliographystyle{plainnat}
% option sectionbib: section rather than chapter

% undefine the cite command to make sure that no coauthor uses it
%\let\cite\undefined

% how to use natbib citations: 
% \citet{SchSmo02} = ``cite in text'', gives Schoelkopf and Smola (2002)
% \citep{SchSmo02} = ``cite in parantheses'', gives (Schoelkopf and Smola, 2002)
% \citealp = ``cite alternative way'', gives Schoelkopf and Smola, 2002


%% APA CITATION STYLE (in the refernece list, year directly after
%% names, not at the end): The translation between commands is as
%% follows
%%\citealp = \citeNP
%%\citet = \citeA
%%\citep = \cite
%% just use the normal natbib commands, here is a translation list: 

%%\usepackage{apacite}
%%\bibliographystyle{apacite}
%%\newcommand{\citealp}[1]{\citeNP{#1}}
%%\newcommand{\citet}[1]{\citeA{#1}}
%%\newcommand{\citep}[1]{\cite{#1}}
%%\renewcommand{\BBAA}{and}
%%\renewcommand{\BCBT}{}
%%\renewcommand{\BTR}{Technical Report}
%%\renewcommand{\BUPhD}{PhD Thesis}
%%\renewcommand{\BPhD}{PhD Thesis}

% \fullciteA -> generates full author list (no et al.)

% ------------------------------------------------------------
% environments: 
% ------------------------------------------------------------

% EQUATION ENVIRONMENTS: 

% abbreviations: \ba = \begin{algin}, \ea = \end{align}
% This cannot be done with a newcommand because of the processing of
% macros in the amslatex package, see tex newsgroup thread ``eeq and amstex''
\def\ba#1\ea{\begin{align*}#1\end{align*}} %\ba = \begin{algin*}, \ea = \end{align*}
\def\banum#1\eanum{\begin{align}#1\end{align}} %\banum = \begin{algin}, \eanum

\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}
\newcommand{\be}{\begin{enumerate}}
\newcommand{\ee}{\end{enumerate}}
\newcommand{\bc}{\begin{center}}
\newcommand{\ec}{\end{center}}

% a list environment with no extra space anywhere (for slides, etc,
% when one has to save space)
\newcommand{\biq}{%bi-quetsch
\begin{list}{$\bullet$}{%
\setlength{\topsep}{0cm}
\setlength{\partopsep}{-\parskip}
\setlength{\leftmargin}{0.8cm}
 \setlength{\itemsep}{0pt}
    \setlength{\parskip}{0pt}
    \setlength{\parsep}{0pt}    
}}
\newcommand{\eiq}{\end{list}}




\def\bv#1\ev{\begin{verbatim}#1\end{verbatim}} %\ba = \begin{algin*}, \ea = \end{align*}

% redefine the labelitemii (default is a dash, this looks like a
% minus). only for non-beamer-documents, in beamer this gives an
% error:
\makeatletter
\@ifclassloaded{beamer}{}{\renewcommand{\labelitemii}{$\bullet$}}
\makeatother




% THEOREM ENVIRONMENTS: 

% now distinguish whether llncs is used or not. if yes, then the
% following commands are already defined, so do not define them again
% (otherwise error message): 
% might be better to look for amsthm, where those things are
% defined. this is sometimes also used in other packages, like beamer


%define theorem environments:
\ifx\lemma\undefined
\typeout{ULE: LEMMA IS UNDEF, THUS DEF IT:}
%define theorem and proof environments:
\newtheorem{example}{Example} 
\newtheorem{theorem}{Theorem} 
\newtheorem{lemma}[theorem]{Lemma} 
\newtheorem{proposition}[theorem]{Proposition} 
\newtheorem{remark}[theorem]{Remark}
%\newtheorem{theorem}[theorem]{Theorem} 
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{heuristic}[theorem]{Heuristic}
\newcounter{ulesexercise}
\newtheorem{exercise}[ulesexercise]{Exercise} %other counter than rest
%
\else
\typeout{ULE: LEMMA IS ALREADY DEFINED }
\fi





% hack for a theorem without number (nn = no number): 
% I define a theorem with a new counter theoremnn. Then I redefine the 
% command which writes the number of this counter to write nothing. 
\newtheorem{theoremnn}{Theorem}
\renewcommand{\thetheoremnn}{\unskip}

% hack for a proposition with a given number: 
\newcounter{dummycounter}
\newtheorem{propcounter}[dummycounter]{Proposition}
% to apply this, set the dummycounter to the value you want, eg 
% \setcounter{dummycounter}{\ref{prop-eps-graph}}
% \addtocounter{dummycounter}{-1} %because will be increased when calling propcounter
% Then call the propcounter. 

% comments in calculations: 
%\newcommand{\comment}[1]{\hspace{1cm}(\text{#1})}



% PROOF ENVIRONMENTS: 
\newenvironment{proofof}[1]{\par\noindent{\em Proof of #1. }}{\hfill\\[2mm]}
\newcommand{\boringqed}{\hfill$\Box$} % unfilled box
\newcommand{\BlackBox}{\rule{1.5ex}{1.5ex}}  % filled black box 
\newcommand{\ulesqed}{\hfill\smiley}

\ifx\proof\undefined
\typeout{ULE: PROOF IS UNDEF, THUS DEF IT:}
\newenvironment{proof}{\par\noindent{\em Proof. }}{\ulesqed\\[2mm]}
\else
\typeout{ULE: PROOF IS ALREADY DEFINED. }
\fi



% ------------------------------------------------------------
% colors
% ------------------------------------------------------------

\input{ules_latex_colors.tex}


% ------------------------------------------------------------
% dealing with pseudocode: 
% ------------------------------------------------------------
% \usepackage[noend]{algorithmic}

% \algsetup{linenosize=\scriptsize\slidegray}
% \algsetup{linenodelimiter=}
% \renewcommand{\algorithmiccomment}[1]{{\small\blue \# #1}}
% \renewcommand{\algorithmicthen}{} % don't want then statements
% \renewcommand{\algorithmicdo}{} % don't want do statements
% \newcommand{\balg}{\begin{algorithmic}[1]}
% \newcommand{\ealg}{\end{algorithmic}}
% \newcommand{\FORL}[2]{% for loop in one line
% \algorithmicfor\ {#1,}\ \algorithmicdo\ {#2,} \;\algorithmicend\ \algorithmicfor\\%
% }
% \newcommand{\IFL}[2]{% for loop in one line
% \STATE{}\algorithmicif\ {(#1),}\ \algorithmicdo\ {#2,} \;\algorithmicend\ \algorithmicif\\%
% }
% \newcommand{\FORALLL}[2]{% forall loop in one line
% \algorithmicforall\ {(#1),}\ \algorithmicdo\ {#2,} \;\algorithmicend\ \algorithmicfor\\%
% }




% ALGORITHM ENVIRONMENT BY FOOT: 

% Usage: \ulesalgorithm{Name of alg}{contents of alg}, see NIPS 2007
% paper...
% nice version by foot is to use: 
% \begin{quote}{ \tt
% ...
% }
% \end{quote}
\newcommand{\ulesalgorithm}[2]{%
\fbox{\parbox{\textwidth}{%
{\bf #1}\\[2mm]
{\tt #2 }
}}
%\vspace{0.5cm}
}



% a similar thing: just moves text a bit to the left (similar to the
% quote environment, but no margin at the right side): 
% use it with \ulesquote{ ... } or perhaps \ulesquote{\texttt ... }
% see stability overview paper at ftml for an example
\newcommand{\ulesquote}[1]{
\begin{list}{}{%
\setlength{\leftmargin}{1cm}%
\setlength{\rightmargin}{0cm}%
%\setlength{\topsep}{0cm}%
}
\item[] {\em #1}
\end{list}
}



% ------------------------------------------------------------
% math letters: 
% ------------------------------------------------------------


\newcommand{\RR}{\mathbb{R}}
\newcommand{\CC}{\mathbb{C}} 
\newcommand{\Nat}{\mathbb{N}} 
\newcommand{\ZZ}{\mathbb{Z}} 
\newcommand{\QQ}{\mathbb{Q}} 
%%  low level versions:  
%%\newcommand{\R}{I\!\!R}
%%\newcommand{\RR}{I\!\!R}
%%\newcommand{\Nat}{I\!\!N} 
%%\newcommand{\CC}{I\!\!\!\!C}


% for compatibility reasons with other people: 
\let\R\undefined %sometimes it is defined as something I don't know
\newcommand{\R}{\RR}
\newcommand{\N}{\Nat}


% note that to generate more curly mathcal symbols i invoked the eucal
% package in the beginning
\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Ccal}{\mathcal{C}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Ecal}{\mathcal{E}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Ical}{\mathcal{I}}
\newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Ocal}{\mathcal{O}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Qcal}{\mathcal{Q}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Scal}{\mathcal{S}}
\newcommand{\Tcal}{\mathcal{T}}
\newcommand{\Ucal}{\mathcal{U}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Wcal}{\mathcal{W}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\Zcal}{\mathcal{Z}}



% ------------------------------------------------------------
% math operators: 
%if they should have limits (such as a sum) use the * version
% ------------------------------------------------------------
% standard stuff: 

\DeclareMathOperator*{\argmin}{argmin} % * falls subscript
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\minimize}{minimize}
\DeclareMathOperator*{\maximize}{maximize}
%\DeclareMathOperator{\aufspan}{span} replace this by linspan ...
\DeclareMathOperator{\linspan}{span}
\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\Cov}{Cov}
\DeclareMathOperator{\Tr}{Tr}% trace
\DeclareMathOperator{\tr}{Tr}% trace
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\supp}{supp} % support of a function
\DeclareMathOperator{\diam}{diam}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\rg}{rg} %range of a funciton
\DeclareMathOperator{\vol}{vol} %volume


%more special stuff: 

\DeclareMathOperator{\rreg}{R_{reg}}
\DeclareMathOperator{\remp}{R_{emp}}
\DeclareMathOperator{\Rreg}{R_{reg}}
\DeclareMathOperator{\Remp}{R_{emp}}
\DeclareMathOperator{\train}{train}
\DeclareMathOperator{\test}{test}
\DeclareMathOperator{\reg}{reg}
%\DeclareMathOperator{\emp}{emp}
\newcommand{\emp}{{\text{emp}}}

\DeclareMathOperator{\Lip}{Lip}

% Norms: Attention, changed. 
% now use them with standard command with curly brackets: 
% \norm{something}
\newcommand{\norm}[1]{\|#1\|}
\newcommand{\norminf}[1]{\|#1\|_{\infty}}
\newcommand{\normone}[1]{\|#1\|_{1}}
\newcommand{\normtwo}[1]{\|#1\|_{2}}
\newcommand{\normltwo}[1]{\|#1\|_{L_2}}
\newcommand{\normltwopn}[1]{\|#1\|_{L_2(P_n)}}
\newcommand{\normltwop}[1]{\|#1\|_{L_2(P_n)}}

% min and max

\newcommand{\pmin}{p_{\min}}
\newcommand{\pmax}{p_{\max}}
\newcommand{\dmin}{d_{\min}}
\newcommand{\dmax}{d_{\max}}
\newcommand{\wmin}{w_{\min}}
\newcommand{\wmax}{w_{\max}}
\newcommand{\rkmin}{R_{k,\min}}
\newcommand{\rkmax}{R_{k,\max}}

% knn stuff: 
\newcommand{\knn}{\ensuremath{\text{kNN}}}
\newcommand{\kNN}{\ensuremath{\text{kNN}}}


% Graph Laplacians: 
\newcommand{\Lsym}{L_{\text{sym}}}
\newcommand{\lsym}{L_{\text{sym}}}
\newcommand{\sym}{_{\text{sym}}}
\newcommand{\Lrw}{L_{\text{rw}}}
\newcommand{\Lun}{L}

%



% Graph cuts and objective functions: 
\DeclareMathOperator{\ratiocut}{RatioCut}
\DeclareMathOperator{\Ratiocut}{RatioCut}
\DeclareMathOperator{\ncut}{Ncut}
\DeclareMathOperator{\Ncut}{Ncut}
\DeclareMathOperator{\cut}{cut}
\DeclareMathOperator{\Cut}{cut}
\DeclareMathOperator{\mincut}{MinCut}
\DeclareMathOperator{\Mincut}{MinCut}
\DeclareMathOperator{\maxcut}{MaxCut}
\DeclareMathOperator{\minmaxcut}{MinMaxCut}
\DeclareMathOperator{\bal}{Balance}

\DeclareMathOperator{\val}{val}
% Landau notation: 

\newcommand{\bigO}{\mathcal{O}}
\newcommand{\BigO}{\bigO}
% the little o is a hack, it is a recaled version of the big0, but we
% need to say how it is supposed to look like in the differnt
% displaystyles: 
\newcommand\littleO{\operatorname{\scriptstyle\mathcal{O}}}
 %  \mathchoice
%   {% \displaystyle
%     \operatorname{\scriptstyle\mathcal{O}}
%   }
%   {% \textstyle
%       \operatorname{\scriptstyle\mathcal{O}}
%   }
%   {% \scriptstyle
%       \operatorname{\scriptscriptstyle\mathcal{O}}
%   }
%   {% \scriptscriptstyle
%       \operatorname{\scalebox{0.8}{$\scriptscriptstyle\mathcal{O}$}}
%   }
% }

% complexity classes: 
\newcommand{\NP}{\ensuremath{\mathbf{NP}}}
\renewcommand{\P}{\ensuremath{\mathbf{P}}}




% ------------------------------------------------------------
% misc math stuff: 
% ------------------------------------------------------------

% various symbols: 

\newcommand{\eps}{\ensuremath{\varepsilon}}
\renewcommand{\epsilon}{\ensuremath{\varepsilon}}
\renewcommand{\phi}{\ensuremath{\varphi}}
%\newcommand{\charfct}{\ensuremath{\text{\bbfamily{1}}}} % hack
\newcommand{\charfct}{\mathbb{1}}
\newcommand{\constantfct}{\mathbf{1}}% constant 1-function
\newcommand{\onevec}{\mathbf{1}}% constant 1-function
\newcommand{\Id}{{I}}% identity matrix 
\newcommand{\id}{\Id}% identity matrix 
\newcommand{\nullfct}{{\bf 0}}
\newcommand{\preperp}[1]{{^\perp}#1} % orthogonal-sign in left upper corner of something
\newcommand{\uniondis}{\mathaccent\cdot\cup}  %disjoint union
\newcommand{\union}{\cup}  
%\newcommand{\entspricht}{\widehat{=}}
\newcommand{\entspricht}{\stackrel{\scriptscriptstyle\wedge}{=}}
\newcommand{\blitz}{\lightning} %widerspruch im beweis. nicht in maths
                                %environment benutzen! 
\newcommand{\widerspruch}{\lightning} %widerspruch im beweis, nicht in maths
                                %environment benutzen! 
\newcommand{\contradition}{\lightning} %widerspruch im beweis, nicht in maths
                                %environment benutzen! 


% probability stuff: 

\newcommand{\as}{a.s.\xspace}
\newcommand{\condon}{\; \big| \;}%conditional on ...
\newcommand{\comma}{\; , \;}%conditional on ...
%\newcommand{\prob}{\mathbb{P}} %probability, the french way
%\newcommand{\expectation}{\mathbb{E}} %expectation, the french way;
\let\Pr\undefined %is defined as something I don't know
\DeclareMathOperator{\Pr}{Pr}


\newcommand{\hd}{\hdots}

%Convergence: 
\newcommand{\tocc}{  \overset{cc}{\to}  }%collectively compact
\newcommand{\tocompact}{  \overset{c}{\to}  }% compact
\newcommand{\topointwise}{  \overset{p}{\to}  }%pointwise
\newcommand{\tonorm}{  \overset{\norm}{\to}  }%in norm
\newcommand{\toplusminus}{ \overset{+-}{\to}  }%up to a change of sign

\newcommand{\CX}{C(\Xcal)} %continuous fct space

% spectral stuff: 
\newcommand{\sigmaess}{\sigma_{\text{ess}}} %essential spectrum
\newcommand{\sigmad}{\sigma_{\text{d}}} %discrete spectrum

% vertical and horizontal vectors, to be used either in text or in
% math mode formulas: 
\newcommand{\tvec}[2]{\ensuremath{\bigl(\begin{smallmatrix}#1\\#2\end{smallmatrix}\bigr)}}%text, vertical
\newcommand{\fvec}[2]{\begin{pmatrix}#1\\#2\end{pmatrix}} %formulas,vertical



% inverting: 
\newcommand{\inv}{^{-1}} %inverse
\newcommand{\pinv}{^{\dagger}} %pseudo-inverse



% ------------------------------------------------------------
% misc non-math: 
% ------------------------------------------------------------
%\newcommand{\maketilde}{\raisebox{0.4ex}{\tiny $\sim$}} % for ~ in
%urls, http addresses
% use \symbol{126} instead
% empty line in a slide: 
%\newcommand{\emptyline}{\bigskip}%is a bit less than an empty line
\newcommand{\emptyline}{\vspace*{0.4cm}} %vspace* also works at beginning of page
\newcommand{\el}{\emptyline}

% for easier references: 
\newcommand{\fig}[1]{Figure~\protect\ref{#1}}
\newcommand{\tab}[1]{Table~\protect\ref{#1}}
\newcommand{\chap}[1]{Chapter~\protect\ref{#1}}
\renewcommand{\sec}[1]{Section~\protect\ref{#1}}
\newcommand{\app}[1]{Appendix~\protect\ref{#1}}
\newcommand{\eq}[1]{Equation~\protect(\ref{#1})}
\newcommand{\pag}[1]{page \protect\pageref{#1}}

\newcommand{\prop}[1]{Proposition~\protect\ref{#1}}
%\newcommand{\coro}[1]{Corollary~\protect\ref{#1}}
%\newcommand{\rema}[1]{Remark~\protect\ref{#1}}
%\newcommand{\exam}[1]{Example~\protect\ref{#1}}
%\newcommand{\appl}[1]{Application~\protect\ref{#1}}
%\newcommand{\algo}[1]{Algorithm~\protect\ref{#1}}
\renewcommand{\th}[1]{Theorem~\protect\ref{#1}}

\newcommand{\ER}{Erd\H{o}s-R\'{e}nyi\xspace} % Erdoes-Renyi in correct spelling
\newcommand{\er}{Erd\H{o}s-R\'{e}nyi\xspace}



\newcommand{\incl}[2]{\hfill\includegraphics[width=#1\textwidth]{#2}\hfill} %width
\newcommand{\inclh}[2]{\hfill\includegraphics[height=#1\textheight]{#2}\hfill} %height
\newcommand{\inclw}[2]{\hfill\includegraphics[width=#1\textwidth]{#2}\hfill} %height


% footnote without any marker: 
\newcommand{\footnoteNoMarker}[1]{%creates a footnote without any marker
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}


% ------------------------------------------------------------
% blob commands: NOW REPLACED BY \biq, \eiq 
% ------------------------------------------------------------

% DO NOT USE IT ANY MORE, JUST KEEP IT FOR CONSISTENCY WITH OLD LATEX
% FILES: 

\newcommand{\blob}{\mbox{}\\[1mm]\mbox{}\hspace{1mm}$\bullet$ } 
% \newcommand{\blobblob}{\mbox{}\\[1mm]\mbox{}\hspace{5mm} $\circ$ } 

% % as in \itemize, with correct indentation over several lines, 
% % without any extra space on top or bottom. call with \blobb{argument}
% \newcommand{\blobb}[1]{%
% \begin{list}{$\bullet$}{%
% \setlength{\topsep}{0cm}
% %\setlength{\partopsep}{-\parskip}
% \setlength{\leftmargin}{0.5cm}
% }{\item #1}%
% \end{list}
% }


% % as in \itemize, with correct indentation over several lines, 
% % without any extra space on top or bottom. call with \blobb{argument}
% \newcommand{\blobblobb}[1]{%
% \begin{list}{$\circ$}{%
% \setlength{\topsep}{0cm}
% %\setlength{\partopsep}{-\parskip}
% \setlength{\leftmargin}{1.1cm}
% }{\item #1}%
% \end{list}
% }
% \newcommand{\bb}[1]{\blobblobb{#1}}
% \newcommand{\blbo}{\blob} %because of constant typo :-)
% %\newcommand{\emptyblob}{\hspace*{0.4cm}}
% %\newcommand{\strich}{\mbox{}\\ - }


% ------------------------------------------------------------
% manuscript preparation phase: 
% ------------------------------------------------------------
\renewcommand{\comment}[1]{{\marginpar{\footnotesize #1}}}
%For switching comments off:
%\newcommand{\comment}[1]{{\mbox{ }}}


% ------------------------------------------------------------
% about the smileys... and wasysym: 
% ------------------------------------------------------------

% because of inconsistent spelling (smiley but frownie)
\newcommand{\smilie}{\smiley}
\newcommand{\neutralface}{\mbox{\small \ensuremath{\bigcirc \hspace{-0.38cm}\sim}}}

% to get rid of a font warning for bold math fonts I don't even use:
% (write each font size which occurs in <size> to suppress warning)
\wasyfamily
\DeclareFontShape{U}{wasy}{b}{n}{ <-10> ssub * wasy/m/n
<10> <10.95> <12> <14.4> <17.28> <20.74> <24.88>wasyb10 }{}

% to produce arbitrary large smileys with wasysym: 
% add the font sizes i want in the end (here: 40, 50, and 60). Then
% can be called with {\fontsize{40}{1} \smiley}: 
\DeclareFontShape{U}{wasy}{m}{n}{ <5> <6> <7> <8> <9> gen * wasy
<10> <10.95> <12> <14.4> <17.28> <20.74> <24.88> <35> <40> <50> <60> wasy10  }{}


% date command (in case one wants to have it consistent over several
% documents, eg in application documents} 
\newcommand{\ulesdateEnglish}{\today}
\newcommand{\ulesdateGerman}{\today} 
% to force a date to be in german: 
%\usepackage[american]{babel} 
%{\selectlanguage{german}\today}



% ------------------------------------------------------------
% propositions, theorems on slides: 
% ------------------------------------------------------------

% proposition environments etc: 
\newcounter{ulestheorem}

% ulesblock is defined in beamerthemeule

% Usage: \ulestheorem{label}{title}{body}
\newcommand{\ulestheorem}[3]{%
\refstepcounter{ulestheorem}%
\begin{ulesblock}{%
Theorem \arabic{ulestheorem}
\label{#1}%
\ifthenelse{\equal{#2}{}}{}{(#2)}}%title of the theorem, if exists
#3 % body of the theorem
\end{ulesblock}%
}

% Usage: \ulestheorem{label}{title}{body}
\newcommand{\ulesproposition}[3]{%
\refstepcounter{ulestheorem}%
\begin{ulesblock}{%
Proposition \arabic{ulestheorem}
\label{#1}%
\ifthenelse{\equal{#2}{}}{}{(#2)}}%title of the theorem, if exists
#3 % body of the theorem
\end{ulesblock}%
}
% Usage: \ulestheorem{label}{title}{body}
\newcommand{\ulescorollary}[3]{%
\refstepcounter{ulestheorem}%
\begin{ulesblock}{%
Corollary \arabic{ulestheorem}
\label{#1}%
\ifthenelse{\equal{#2}{}}{}{(#2)}}%title of the theorem, if exists
#3 % body of the theorem
\end{ulesblock}%
}

